Prompt Compression via Activation Aggregation

Large language models process prompts by propagating activations through dozens of layers before generating a response. We ask whether the task-relevant information contained in an instruction prompt can be compressed into a single activation vector and re-injected into the model, replacing the original token sequence? We show this is achievable using a learned weighted sum of activations extracted at an intermediate layer and injected at an early layer of the target LLM. The compressed vector preserves task-relevant information, incurring an accuracy drop of under $2\%$ relative to full prompt processing. Beyond its practical implications, including reducing per-query computation for fixed instruction prompts without reprocessing the original token sequence, our analysis reveals structure in the activation space of LLMs: (i) mid-layer representations transfer meaningfully to early layers, suggesting a degree of cross-layer compatibility in how information is encoded; (ii) a single activation vector encodes a quantifiable and recoverable amount of semantic information; (iii) a weighted sum of activations is a robust representation compressor.

==> figures/weighted_texts/token_weights.berlin_clubs.kl_divergences.tex <==
% ── Token weight visualization ─────────────────────────────────────
% Required packages: xcolor
\setlength{\fboxsep}{1pt}

% Color definitions
\definecolor{tc0}{RGB}{242,157,109}
\definecolor{tc1}{RGB}{244,174,135}
\definecolor{tc2}{RGB}{244,175,135}
\definecolor{tc3}{RGB}{243,166,122}
\definecolor{tc4}{RGB}{244,173,132}
\definecolor{tc5}{RGB}{243,166,122}
\definecolor{tc6}{RGB}{245,177,138}
\definecolor{tc7}{RGB}{244,170,128}
\definecolor{tc8}{RGB}{242,159,112}
\definecolor{tc9}{RGB}{246,188,156}
\definecolor{tc10}{RGB}{246,184,150}

% Tokens
\noindent
{\color{black}\colorbox{tc0}{\strut \small Do}}%
{\color{black}\colorbox{tc1}{\strut \small  Berlin}}%
{\color{black}\colorbox{tc2}{\strut \small  clubs}}%
{\color{black}\colorbox{tc3}{\strut \small  turn}}%
{\color{black}\colorbox{tc4}{\strut \small  down}}%
{\color{black}\colorbox{tc5}{\strut \small  the}}%
{\color{black}\colorbox{tc6}{\strut \small  music}}%
{\color{black}\colorbox{tc7}{\strut \small  during}}%
{\color{black}\colorbox{tc8}{\strut \small  the}}%
{\color{black}\colorbox{tc9}{\strut \small  week}}%
{\color{black}\colorbox{tc10}{\strut \small ?}}
% ────────────────────────────────────────────────────────────────────

==> figures/weighted_texts/token_weights.berlin_clubs.similarities.tex <==
% ── Token weight visualization ─────────────────────────────────────
% Required packages: xcolor
\setlength{\fboxsep}{1pt}

% Color definitions
\definecolor{tc0}{RGB}{251,226,212}
\definecolor{tc1}{RGB}{244,174,134}
\definecolor{tc2}{RGB}{245,178,140}
\definecolor{tc3}{RGB}{247,198,171}
\definecolor{tc4}{RGB}{247,195,166}
\definecolor{tc5}{RGB}{252,229,217}
\definecolor{tc6}{RGB}{245,181,144}
\definecolor{tc7}{RGB}{248,199,172}
\definecolor{tc8}{RGB}{254,246,241}
\definecolor{tc9}{RGB}{242,157,109}
\definecolor{tc10}{RGB}{242,158,110}

% Tokens
\noindent
{\color{black}\colorbox{tc0}{\strut \small Do}}%
{\color{black}\colorbox{tc1}{\strut \small  Berlin}}%
{\color{black}\colorbox{tc2}{\strut \small  clubs}}%
{\color{black}\colorbox{tc3}{\strut \small  turn}}%
{\color{black}\colorbox{tc4}{\strut \small  down}}%
{\color{black}\colorbox{tc5}{\strut \small  the}}%
{\color{black}\colorbox{tc6}{\strut \small  music}}%
{\color{black}\colorbox{tc7}{\strut \small  during}}%
{\color{black}\colorbox{tc8}{\strut \small  the}}%
{\color{black}\colorbox{tc9}{\strut \small  week}}%
{\color{black}\colorbox{tc10}{\strut \small ?}}
% ────────────────────────────────────────────────────────────────────

==> figures/weighted_texts/token_weights.berlin_clubs.weights.tex <==
% ── Token weight visualization ─────────────────────────────────────
% Required packages: xcolor
\setlength{\fboxsep}{1pt}

% Color definitions
\definecolor{tc0}{RGB}{251,222,205}
\definecolor{tc1}{RGB}{243,163,118}
\definecolor{tc2}{RGB}{248,203,177}
\definecolor{tc3}{RGB}{211,215,226}
\definecolor{tc4}{RGB}{250,217,198}
\definecolor{tc5}{RGB}{254,251,249}
\definecolor{tc6}{RGB}{246,186,152}
\definecolor{tc7}{RGB}{252,232,220}
\definecolor{tc8}{RGB}{1,25,89}
\definecolor{tc9}{RGB}{242,157,109}
\definecolor{tc10}{RGB}{244,171,130}

% Tokens
\noindent
{\color{black}\colorbox{tc0}{\strut \small Do}}%
{\color{black}\colorbox{tc1}{\strut \small  Berlin}}%
{\color{black}\colorbox{tc2}{\strut \small  clubs}}%
{\color{black}\colorbox{tc3}{\strut \small  turn}}%
{\color{black}\colorbox{tc4}{\strut \small  down}}%
{\color{black}\colorbox{tc5}{\strut \small  the}}%
{\color{black}\colorbox{tc6}{\strut \small  music}}%
{\color{black}\colorbox{tc7}{\strut \small  during}}%
{\color{white}\colorbox{tc8}{\strut \small  the}}%
{\color{black}\colorbox{tc9}{\strut \small  week}}%
{\color{black}\colorbox{tc10}{\strut \small ?}}
% ────────────────────────────────────────────────────────────────────

==> figures/weighted_texts/token_weights.bones_questions.kl_divergences.tex <==
% ── Token weight visualization ─────────────────────────────────────
% Required packages: xcolor
\setlength{\fboxsep}{1pt}

% Color definitions
\definecolor{tc0}{RGB}{244,174,135}
\definecolor{tc1}{RGB}{243,167,124}
\definecolor{tc2}{RGB}{242,157,109}
\definecolor{tc3}{RGB}{246,190,157}
\definecolor{tc4}{RGB}{248,205,180}
\definecolor{tc5}{RGB}{246,189,157}
\definecolor{tc6}{RGB}{246,188,156}
\definecolor{tc7}{RGB}{244,171,130}
\definecolor{tc8}{RGB}{245,176,137}
\definecolor{tc9}{RGB}{246,186,153}
\definecolor{tc10}{RGB}{247,191,160}
\definecolor{tc11}{RGB}{246,189,157}
\definecolor{tc12}{RGB}{247,197,169}
\definecolor{tc13}{RGB}{249,213,193}

% Tokens
\noindent
{\color{black}\colorbox{tc0}{\strut \small What}}%
{\color{black}\colorbox{tc1}{\strut \small  is}}%
{\color{black}\colorbox{tc2}{\strut \small  the}}%
{\color{black}\colorbox{tc3}{\strut \small  body}}%
{\color{black}\colorbox{tc4}{\strut \small  part}}%
{\color{black}\colorbox{tc5}{\strut \small  in}}%
{\color{black}\colorbox{tc6}{\strut \small  which}}%
{\color{black}\colorbox{tc7}{\strut \small  the}}%
{\color{black}\colorbox{tc8}{\strut \small  Pat}}%
{\color{black}\colorbox{tc9}{\strut \small ella}}%
{\color{black}\colorbox{tc10}{\strut \small  bone}}%
{\color{black}\colorbox{tc11}{\strut \small  is}}%
{\color{black}\colorbox{tc12}{\strut \small  located}}%
{\color{black}\colorbox{tc13}{\strut \small ?}}
% ────────────────────────────────────────────────────────────────────

==> figures/weighted_texts/token_weights.bones_questions.similarities.tex <==
% ── Token weight visualization ─────────────────────────────────────
% Required packages: xcolor
\setlength{\fboxsep}{1pt}

% Color definitions
\definecolor{tc0}{RGB}{253,241,234}
\definecolor{tc1}{RGB}{149,159,186}
\definecolor{tc2}{RGB}{1,25,89}
\definecolor{tc3}{RGB}{249,212,191}
\definecolor{tc4}{RGB}{244,174,135}
\definecolor{tc5}{RGB}{249,211,189}
\definecolor{tc6}{RGB}{249,210,189}
\definecolor{tc7}{RGB}{254,249,246}
\definecolor{tc8}{RGB}{252,234,224}
\definecolor{tc9}{RGB}{249,206,183}
\definecolor{tc10}{RGB}{247,197,168}
\definecolor{tc11}{RGB}{248,202,176}
\definecolor{tc12}{RGB}{246,190,158}
\definecolor{tc13}{RGB}{242,157,109}

% Tokens
\noindent
{\color{black}\colorbox{tc0}{\strut \small What}}%
{\color{white}\colorbox{tc1}{\strut \small  is}}%
{\color{white}\colorbox{tc2}{\strut \small  the}}%
{\color{black}\colorbox{tc3}{\strut \small  body}}%
{\color{black}\colorbox{tc4}{\strut \small  part}}%
{\color{black}\colorbox{tc5}{\strut \small  in}}%
{\color{black}\colorbox{tc6}{\strut \small  which}}%
{\color{black}\colorbox{tc7}{\strut \small  the}}%
{\color{black}\colorbox{tc8}{\strut \small  Pat}}%
{\color{black}\colorbox{tc9}{\strut \small ella}}%
{\color{black}\colorbox{tc10}{\strut \small  bone}}%
{\color{black}\colorbox{tc11}{\strut \small  is}}%
{\color{black}\colorbox{tc12}{\strut \small  located}}%
{\color{black}\colorbox{tc13}{\strut \small ?}}
% ────────────────────────────────────────────────────────────────────

==> figures/weighted_texts/token_weights.bones_questions.weights.tex <==
% ── Token weight visualization ─────────────────────────────────────
% Required packages: xcolor
\setlength{\fboxsep}{1pt}

% Color definitions
\definecolor{tc0}{RGB}{249,211,190}
\definecolor{tc1}{RGB}{146,157,184}
\definecolor{tc2}{RGB}{1,25,89}
\definecolor{tc3}{RGB}{250,221,204}
\definecolor{tc4}{RGB}{243,163,118}
\definecolor{tc5}{RGB}{251,228,215}
\definecolor{tc6}{RGB}{253,240,232}
\definecolor{tc7}{RGB}{100,115,154}
\definecolor{tc8}{RGB}{185,191,209}
\definecolor{tc9}{RGB}{249,213,192}
\definecolor{tc10}{RGB}{249,208,185}
\definecolor{tc11}{RGB}{251,226,211}
\definecolor{tc12}{RGB}{249,208,185}
\definecolor{tc13}{RGB}{242,157,109}

% Tokens
\noindent
{\color{black}\colorbox{tc0}{\strut \small What}}%
{\color{white}\colorbox{tc1}{\strut \small  is}}%
{\color{white}\colorbox{tc2}{\strut \small  the}}%
{\color{black}\colorbox{tc3}{\strut \small  body}}%
{\color{black}\colorbox{tc4}{\strut \small  part}}%
{\color{black}\colorbox{tc5}{\strut \small  in}}%
{\color{black}\colorbox{tc6}{\strut \small  which}}%
{\color{white}\colorbox{tc7}{\strut \small  the}}%
{\color{black}\colorbox{tc8}{\strut \small  Pat}}%
{\color{black}\colorbox{tc9}{\strut \small ella}}%
{\color{black}\colorbox{tc10}{\strut \small  bone}}%
{\color{black}\colorbox{tc11}{\strut \small  is}}%
{\color{black}\colorbox{tc12}{\strut \small  located}}%
{\color{black}\colorbox{tc13}{\strut \small ?}}
% ────────────────────────────────────────────────────────────────────

==> figures/weighted_texts/token_weights.harry_potter_long_prompt.kl_divergences.tex <==
% ── Token weight visualization ─────────────────────────────────────
% Required packages: xcolor
\setlength{\fboxsep}{1pt}

% Color definitions
\definecolor{tc0}{RGB}{243,168,125}
\definecolor{tc1}{RGB}{244,168,126}
\definecolor{tc2}{RGB}{244,168,126}
\definecolor{tc3}{RGB}{245,176,138}
\definecolor{tc4}{RGB}{243,162,117}
\definecolor{tc5}{RGB}{243,162,117}
\definecolor{tc6}{RGB}{245,178,141}
\definecolor{tc7}{RGB}{246,185,150}
\definecolor{tc8}{RGB}{244,174,134}
\definecolor{tc9}{RGB}{243,166,122}
\definecolor{tc10}{RGB}{242,160,114}
\definecolor{tc11}{RGB}{242,160,114}
\definecolor{tc12}{RGB}{242,157,109}
\definecolor{tc13}{RGB}{242,159,112}
\definecolor{tc14}{RGB}{245,178,141}
\definecolor{tc15}{RGB}{243,164,119}
\definecolor{tc16}{RGB}{243,163,117}
\definecolor{tc17}{RGB}{245,177,139}
\definecolor{tc18}{RGB}{244,175,136}
\definecolor{tc19}{RGB}{243,167,124}
\definecolor{tc20}{RGB}{244,169,126}
\definecolor{tc21}{RGB}{243,165,120}
\definecolor{tc22}{RGB}{244,172,131}
\definecolor{tc23}{RGB}{243,164,119}
\definecolor{tc24}{RGB}{245,177,139}
\definecolor{tc25}{RGB}{246,187,154}
\definecolor{tc26}{RGB}{246,184,150}
\definecolor{tc27}{RGB}{245,181,145}
\definecolor{tc28}{RGB}{245,177,138}
\definecolor{tc29}{RGB}{245,179,142}
\definecolor{tc30}{RGB}{245,182,146}
\definecolor{tc31}{RGB}{246,185,151}
\definecolor{tc32}{RGB}{244,176,137}
\definecolor{tc33}{RGB}{244,170,129}
\definecolor{tc34}{RGB}{243,168,126}
\definecolor{tc35}{RGB}{244,175,136}
\definecolor{tc36}{RGB}{245,177,139}
\definecolor{tc37}{RGB}{245,180,143}
\definecolor{tc38}{RGB}{245,181,145}
\definecolor{tc39}{RGB}{246,186,152}
\definecolor{tc40}{RGB}{245,179,142}
\definecolor{tc41}{RGB}{244,174,134}
\definecolor{tc42}{RGB}{244,175,135}
\definecolor{tc43}{RGB}{244,172,131}
\definecolor{tc44}{RGB}{244,175,136}
\definecolor{tc45}{RGB}{246,187,154}
\definecolor{tc46}{RGB}{245,180,144}
\definecolor{tc47}{RGB}{246,185,151}
\definecolor{tc48}{RGB}{246,188,156}
\definecolor{tc49}{RGB}{245,179,142}
\definecolor{tc50}{RGB}{245,177,139}
\definecolor{tc51}{RGB}{245,178,140}
\definecolor{tc52}{RGB}{245,179,142}
\definecolor{tc53}{RGB}{245,179,141}
\definecolor{tc54}{RGB}{245,180,144}
\definecolor{tc55}{RGB}{245,181,145}
\definecolor{tc56}{RGB}{245,180,143}
\definecolor{tc57}{RGB}{246,189,157}
\definecolor{tc58}{RGB}{246,190,159}

% Tokens
\noindent
{\color{black}\colorbox{tc0}{\strut \small Mr}}%
{\color{black}\colorbox{tc1}{\strut \small .}}%
{\color{black}\colorbox{tc2}{\strut \small  and}}%
{\color{black}\colorbox{tc3}{\strut \small  Mrs}}%
{\color{black}\colorbox{tc4}{\strut \small .}}%
{\color{black}\colorbox{tc5}{\strut \small  D}}%
{\color{black}\colorbox{tc6}{\strut \small urs}}%
{\color{black}\colorbox{tc7}{\strut \small ley}}%
{\color{black}\colorbox{tc8}{\strut \small ,}}%
{\color{black}\colorbox{tc9}{\strut \small  of}}%
{\color{black}\colorbox{tc10}{\strut \small  number}}%
{\color{black}\colorbox{tc11}{\strut \small  four}}%
{\color{black}\colorbox{tc12}{\strut \small ,}}%
{\color{black}\colorbox{tc13}{\strut \small  Priv}}%
{\color{black}\colorbox{tc14}{\strut \small et}}%
{\color{black}\colorbox{tc15}{\strut \small  Drive}}%
{\color{black}\colorbox{tc16}{\strut \small ,}}%
{\color{black}\colorbox{tc17}{\strut \small  were}}%
{\color{black}\colorbox{tc18}{\strut \small  proud}}%
{\color{black}\colorbox{tc19}{\strut \small  to}}%
{\color{black}\colorbox{tc20}{\strut \small  say}}%
{\color{black}\colorbox{tc21}{\strut \small  that}}%
{\color{black}\colorbox{tc22}{\strut \small  they}}%
{\color{black}\colorbox{tc23}{\strut \small  were}}%
{\color{black}\colorbox{tc24}{\strut \small  perfectly}}%
{\color{black}\colorbox{tc25}{\strut \small  normal}}%
{\color{black}\colorbox{tc26}{\strut \small ,}}%
{\color{black}\colorbox{tc27}{\strut \small  thank}}%
{\color{black}\colorbox{tc28}{\strut \small  you}}%
{\color{black}\colorbox{tc29}{\strut \small  very}}%
{\color{black}\colorbox{tc30}{\strut \small  much}}%
{\color{black}\colorbox{tc31}{\strut \small .}}%
{\color{black}\colorbox{tc32}{\strut \small  They}}%
{\color{black}\colorbox{tc33}{\strut \small  were}}%
{\color{black}\colorbox{tc34}{\strut \small  the}}%
{\color{black}\colorbox{tc35}{\strut \small  last}}%
{\color{black}\colorbox{tc36}{\strut \small  people}}%
{\color{black}\colorbox{tc37}{\strut \small  you}}%
{\color{black}\colorbox{tc38}{\strut \small 'd}}%
{\color{black}\colorbox{tc39}{\strut \small  expect}}%
{\color{black}\colorbox{tc40}{\strut \small  to}}%
{\color{black}\colorbox{tc41}{\strut \small  be}}%
{\color{black}\colorbox{tc42}{\strut \small  involved}}%
{\color{black}\colorbox{tc43}{\strut \small  in}}%
{\color{black}\colorbox{tc44}{\strut \small  anything}}%
{\color{black}\colorbox{tc45}{\strut \small  strange}}%
{\color{black}\colorbox{tc46}{\strut \small  or}}%
{\color{black}\colorbox{tc47}{\strut \small  mysterious}}%
{\color{black}\colorbox{tc48}{\strut \small ,}}%
{\color{black}\colorbox{tc49}{\strut \small  because}}%
{\color{black}\colorbox{tc50}{\strut \small  they}}%
{\color{black}\colorbox{tc51}{\strut \small  just}}%
{\color{black}\colorbox{tc52}{\strut \small  didn}}%
{\color{black}\colorbox{tc53}{\strut \small 't}}%
{\color{black}\colorbox{tc54}{\strut \small  hold}}%
{\color{black}\colorbox{tc55}{\strut \small  with}}%
{\color{black}\colorbox{tc56}{\strut \small  such}}%
{\color{black}\colorbox{tc57}{\strut \small  nonsense}}%
{\color{black}\colorbox{tc58}{\strut \small .}}
% ────────────────────────────────────────────────────────────────────

==> figures/weighted_texts/token_weights.harry_potter_long_prompt.similarities.tex <==
% ── Token weight visualization ─────────────────────────────────────
% Required packages: xcolor
\setlength{\fboxsep}{1pt}

% Color definitions
\definecolor{tc0}{RGB}{250,221,204}
\definecolor{tc1}{RGB}{254,247,243}
\definecolor{tc2}{RGB}{252,234,223}
\definecolor{tc3}{RGB}{250,220,203}
\definecolor{tc4}{RGB}{104,118,156}
\definecolor{tc5}{RGB}{86,102,144}
\definecolor{tc6}{RGB}{250,218,200}
\definecolor{tc7}{RGB}{247,197,168}
\definecolor{tc8}{RGB}{252,230,218}
\definecolor{tc9}{RGB}{254,249,247}
\definecolor{tc10}{RGB}{135,147,177}
\definecolor{tc11}{RGB}{64,82,130}
\definecolor{tc12}{RGB}{1,25,89}
\definecolor{tc13}{RGB}{61,80,128}
\definecolor{tc14}{RGB}{252,230,217}
\definecolor{tc15}{RGB}{191,197,213}
\definecolor{tc16}{RGB}{137,148,178}
\definecolor{tc17}{RGB}{251,224,209}
\definecolor{tc18}{RGB}{249,213,192}
\definecolor{tc19}{RGB}{254,251,249}
\definecolor{tc20}{RGB}{253,237,229}
\definecolor{tc21}{RGB}{229,232,238}
\definecolor{tc22}{RGB}{253,238,230}
\definecolor{tc23}{RGB}{197,203,217}
\definecolor{tc24}{RGB}{249,211,189}
\definecolor{tc25}{RGB}{243,167,124}
\definecolor{tc26}{RGB}{246,189,157}
\definecolor{tc27}{RGB}{248,199,171}
\definecolor{tc28}{RGB}{248,204,179}
\definecolor{tc29}{RGB}{249,207,183}
\definecolor{tc30}{RGB}{246,189,156}
\definecolor{tc31}{RGB}{245,178,141}
\definecolor{tc32}{RGB}{250,215,195}
\definecolor{tc33}{RGB}{252,230,218}
\definecolor{tc34}{RGB}{254,249,246}
\definecolor{tc35}{RGB}{251,226,211}
\definecolor{tc36}{RGB}{251,223,208}
\definecolor{tc37}{RGB}{248,203,178}
\definecolor{tc38}{RGB}{248,203,177}
\definecolor{tc39}{RGB}{246,185,151}
\definecolor{tc40}{RGB}{250,221,204}
\definecolor{tc41}{RGB}{253,237,228}
\definecolor{tc42}{RGB}{252,232,221}
\definecolor{tc43}{RGB}{252,231,219}
\definecolor{tc44}{RGB}{249,208,185}
\definecolor{tc45}{RGB}{243,165,121}
\definecolor{tc46}{RGB}{248,200,173}
\definecolor{tc47}{RGB}{245,180,143}
\definecolor{tc48}{RGB}{244,174,135}
\definecolor{tc49}{RGB}{249,212,191}
\definecolor{tc50}{RGB}{249,206,182}
\definecolor{tc51}{RGB}{250,215,195}
\definecolor{tc52}{RGB}{249,210,188}
\definecolor{tc53}{RGB}{248,204,178}
\definecolor{tc54}{RGB}{250,219,201}
\definecolor{tc55}{RGB}{247,193,162}
\definecolor{tc56}{RGB}{248,205,180}
\definecolor{tc57}{RGB}{244,174,134}
\definecolor{tc58}{RGB}{242,157,109}

% Tokens
\noindent
{\color{black}\colorbox{tc0}{\strut \small Mr}}%
{\color{black}\colorbox{tc1}{\strut \small .}}%
{\color{black}\colorbox{tc2}{\strut \small  and}}%
{\color{black}\colorbox{tc3}{\strut \small  Mrs}}%
{\color{white}\colorbox{tc4}{\strut \small .}}%
{\color{white}\colorbox{tc5}{\strut \small  D}}%
{\color{black}\colorbox{tc6}{\strut \small urs}}%
{\color{black}\colorbox{tc7}{\strut \small ley}}%
{\color{black}\colorbox{tc8}{\strut \small ,}}%
{\color{black}\colorbox{tc9}{\strut \small  of}}%
{\color{white}\colorbox{tc10}{\strut \small  number}}%
{\color{white}\colorbox{tc11}{\strut \small  four}}%
{\color{white}\colorbox{tc12}{\strut \small ,}}%
{\color{white}\colorbox{tc13}{\strut \small  Priv}}%
{\color{black}\colorbox{tc14}{\strut \small et}}%
{\color{black}\colorbox{tc15}{\strut \small  Drive}}%
{\color{white}\colorbox{tc16}{\strut \small ,}}%
{\color{black}\colorbox{tc17}{\strut \small  were}}%
{\color{black}\colorbox{tc18}{\strut \small  proud}}%
{\color{black}\colorbox{tc19}{\strut \small  to}}%
{\color{black}\colorbox{tc20}{\strut \small  say}}%
{\color{black}\colorbox{tc21}{\strut \small  that}}%
{\color{black}\colorbox{tc22}{\strut \small  they}}%
{\color{black}\colorbox{tc23}{\strut \small  were}}%
{\color{black}\colorbox{tc24}{\strut \small  perfectly}}%
{\color{black}\colorbox{tc25}{\strut \small  normal}}%
{\color{black}\colorbox{tc26}{\strut \small ,}}%
{\color{black}\colorbox{tc27}{\strut \small  thank}}%
{\color{black}\colorbox{tc28}{\strut \small  you}}%
{\color{black}\colorbox{tc29}{\strut \small  very}}%
{\color{black}\colorbox{tc30}{\strut \small  much}}%
{\color{black}\colorbox{tc31}{\strut \small .}}%
{\color{black}\colorbox{tc32}{\strut \small  They}}%
{\color{black}\colorbox{tc33}{\strut \small  were}}%
{\color{black}\colorbox{tc34}{\strut \small  the}}%
{\color{black}\colorbox{tc35}{\strut \small  last}}%
{\color{black}\colorbox{tc36}{\strut \small  people}}%
{\color{black}\colorbox{tc37}{\strut \small  you}}%
{\color{black}\colorbox{tc38}{\strut \small 'd}}%
{\color{black}\colorbox{tc39}{\strut \small  expect}}%
{\color{black}\colorbox{tc40}{\strut \small  to}}%
{\color{black}\colorbox{tc41}{\strut \small  be}}%
{\color{black}\colorbox{tc42}{\strut \small  involved}}%
{\color{black}\colorbox{tc43}{\strut \small  in}}%
{\color{black}\colorbox{tc44}{\strut \small  anything}}%
{\color{black}\colorbox{tc45}{\strut \small  strange}}%
{\color{black}\colorbox{tc46}{\strut \small  or}}%
{\color{black}\colorbox{tc47}{\strut \small  mysterious}}%
{\color{black}\colorbox{tc48}{\strut \small ,}}%
{\color{black}\colorbox{tc49}{\strut \small  because}}%
{\color{black}\colorbox{tc50}{\strut \small  they}}%
{\color{black}\colorbox{tc51}{\strut \small  just}}%
{\color{black}\colorbox{tc52}{\strut \small  didn}}%
{\color{black}\colorbox{tc53}{\strut \small 't}}%
{\color{black}\colorbox{tc54}{\strut \small  hold}}%
{\color{black}\colorbox{tc55}{\strut \small  with}}%
{\color{black}\colorbox{tc56}{\strut \small  such}}%
{\color{black}\colorbox{tc57}{\strut \small  nonsense}}%
{\color{black}\colorbox{tc58}{\strut \small .}}
% ────────────────────────────────────────────────────────────────────

==> figures/weighted_texts/token_weights.harry_potter_long_prompt.weights.tex <==
% ── Token weight visualization ─────────────────────────────────────
% Required packages: xcolor
\setlength{\fboxsep}{1pt}

% Color definitions
\definecolor{tc0}{RGB}{251,222,206}
\definecolor{tc1}{RGB}{249,207,184}
\definecolor{tc2}{RGB}{250,220,203}
\definecolor{tc3}{RGB}{242,158,111}
\definecolor{tc4}{RGB}{1,25,89}
\definecolor{tc5}{RGB}{63,81,130}
\definecolor{tc6}{RGB}{249,208,185}
\definecolor{tc7}{RGB}{246,186,152}
\definecolor{tc8}{RGB}{252,231,220}
\definecolor{tc9}{RGB}{253,243,236}
\definecolor{tc10}{RGB}{140,151,180}
\definecolor{tc11}{RGB}{254,248,244}
\definecolor{tc12}{RGB}{88,104,146}
\definecolor{tc13}{RGB}{61,80,128}
\definecolor{tc14}{RGB}{251,228,215}
\definecolor{tc15}{RGB}{252,235,226}
\definecolor{tc16}{RGB}{193,199,215}
\definecolor{tc17}{RGB}{253,238,230}
\definecolor{tc18}{RGB}{247,196,167}
\definecolor{tc19}{RGB}{78,95,139}
\definecolor{tc20}{RGB}{252,231,220}
\definecolor{tc21}{RGB}{85,101,144}
\definecolor{tc22}{RGB}{253,242,235}
\definecolor{tc23}{RGB}{124,136,169}
\definecolor{tc24}{RGB}{250,219,201}
\definecolor{tc25}{RGB}{242,157,109}
\definecolor{tc26}{RGB}{250,218,200}
\definecolor{tc27}{RGB}{249,210,189}
\definecolor{tc28}{RGB}{250,218,199}
\definecolor{tc29}{RGB}{250,215,196}
\definecolor{tc30}{RGB}{250,218,200}
\definecolor{tc31}{RGB}{248,201,174}
\definecolor{tc32}{RGB}{252,235,224}
\definecolor{tc33}{RGB}{122,135,168}
\definecolor{tc34}{RGB}{100,114,154}
\definecolor{tc35}{RGB}{251,224,209}
\definecolor{tc36}{RGB}{253,238,230}
\definecolor{tc37}{RGB}{249,211,190}
\definecolor{tc38}{RGB}{250,217,198}
\definecolor{tc39}{RGB}{246,186,152}
\definecolor{tc40}{RGB}{253,238,229}
\definecolor{tc41}{RGB}{231,233,239}
\definecolor{tc42}{RGB}{251,224,209}
\definecolor{tc43}{RGB}{134,146,176}
\definecolor{tc44}{RGB}{143,154,182}
\definecolor{tc45}{RGB}{243,163,117}
\definecolor{tc46}{RGB}{250,219,202}
\definecolor{tc47}{RGB}{248,200,174}
\definecolor{tc48}{RGB}{249,209,187}
\definecolor{tc49}{RGB}{254,248,245}
\definecolor{tc50}{RGB}{251,227,213}
\definecolor{tc51}{RGB}{250,219,201}
\definecolor{tc52}{RGB}{252,232,221}
\definecolor{tc53}{RGB}{251,225,210}
\definecolor{tc54}{RGB}{252,229,217}
\definecolor{tc55}{RGB}{251,225,210}
\definecolor{tc56}{RGB}{252,234,224}
\definecolor{tc57}{RGB}{245,180,143}
\definecolor{tc58}{RGB}{244,169,127}

% Tokens
\noindent
{\color{black}\colorbox{tc0}{\strut \small Mr}}%
{\color{black}\colorbox{tc1}{\strut \small .}}%
{\color{black}\colorbox{tc2}{\strut \small  and}}%
{\color{black}\colorbox{tc3}{\strut \small  Mrs}}%
{\color{white}\colorbox{tc4}{\strut \small .}}%
{\color{white}\colorbox{tc5}{\strut \small  D}}%
{\color{black}\colorbox{tc6}{\strut \small urs}}%
{\color{black}\colorbox{tc7}{\strut \small ley}}%
{\color{black}\colorbox{tc8}{\strut \small ,}}%
{\color{black}\colorbox{tc9}{\strut \small  of}}%
{\color{white}\colorbox{tc10}{\strut \small  number}}%
{\color{black}\colorbox{tc11}{\strut \small  four}}%
{\color{white}\colorbox{tc12}{\strut \small ,}}%
{\color{white}\colorbox{tc13}{\strut \small  Priv}}%
{\color{black}\colorbox{tc14}{\strut \small et}}%
{\color{black}\colorbox{tc15}{\strut \small  Drive}}%
{\color{black}\colorbox{tc16}{\strut \small ,}}%
{\color{black}\colorbox{tc17}{\strut \small  were}}%
{\color{black}\colorbox{tc18}{\strut \small  proud}}%
{\color{white}\colorbox{tc19}{\strut \small  to}}%
{\color{black}\colorbox{tc20}{\strut \small  say}}%
{\color{white}\colorbox{tc21}{\strut \small  that}}%
{\color{black}\colorbox{tc22}{\strut \small  they}}%
{\color{white}\colorbox{tc23}{\strut \small  were}}%
{\color{black}\colorbox{tc24}{\strut \small  perfectly}}%
{\color{black}\colorbox{tc25}{\strut \small  normal}}%
{\color{black}\colorbox{tc26}{\strut \small ,}}%
{\color{black}\colorbox{tc27}{\strut \small  thank}}%
{\color{black}\colorbox{tc28}{\strut \small  you}}%
{\color{black}\colorbox{tc29}{\strut \small  very}}%
{\color{black}\colorbox{tc30}{\strut \small  much}}%
{\color{black}\colorbox{tc31}{\strut \small .}}%
{\color{black}\colorbox{tc32}{\strut \small  They}}%
{\color{white}\colorbox{tc33}{\strut \small  were}}%
{\color{white}\colorbox{tc34}{\strut \small  the}}%
{\color{black}\colorbox{tc35}{\strut \small  last}}%
{\color{black}\colorbox{tc36}{\strut \small  people}}%
{\color{black}\colorbox{tc37}{\strut \small  you}}%
{\color{black}\colorbox{tc38}{\strut \small 'd}}%
{\color{black}\colorbox{tc39}{\strut \small  expect}}%
{\color{black}\colorbox{tc40}{\strut \small  to}}%
{\color{black}\colorbox{tc41}{\strut \small  be}}%
{\color{black}\colorbox{tc42}{\strut \small  involved}}%
{\color{white}\colorbox{tc43}{\strut \small  in}}%
{\color{white}\colorbox{tc44}{\strut \small  anything}}%
{\color{black}\colorbox{tc45}{\strut \small  strange}}%
{\color{black}\colorbox{tc46}{\strut \small  or}}%
{\color{black}\colorbox{tc47}{\strut \small  mysterious}}%
{\color{black}\colorbox{tc48}{\strut \small ,}}%
{\color{black}\colorbox{tc49}{\strut \small  because}}%
{\color{black}\colorbox{tc50}{\strut \small  they}}%
{\color{black}\colorbox{tc51}{\strut \small  just}}%
{\color{black}\colorbox{tc52}{\strut \small  didn}}%
{\color{black}\colorbox{tc53}{\strut \small 't}}%
{\color{black}\colorbox{tc54}{\strut \small  hold}}%
{\color{black}\colorbox{tc55}{\strut \small  with}}%
{\color{black}\colorbox{tc56}{\strut \small  such}}%
{\color{black}\colorbox{tc57}{\strut \small  nonsense}}%
{\color{black}\colorbox{tc58}{\strut \small .}}
% ────────────────────────────────────────────────────────────────────
